DataLens: ML-Oriented Interactive Tabular Data Quality Dashboard

Maintaining high data quality is crucial for reliable data analysis and machine learning (ML). However, existing data quality management tools often lack automation, interactivity, and integration with ML workflows. This demonstration paper introduces DataLens, a novel interactive dashboard designed to streamline and automate the data quality management process for tabular data. DataLens integrates a suite of data profiling, error detection, and repair tools, including statistical, rule-based, and ML-based methods. It features a user-in-the-loop module for interactive rule validation, data labeling, and custom rule definition, enabling domain experts to guide the cleaning process. Furthermore, DataLens implements an iterative cleaning module that automatically selects optimal cleaning tools based on downstream ML model performance. To ensure reproducibility, DataLens generates DataSheets capturing essential metadata and integrates with MLflow and Delta Lake for experiment tracking and data version control. This demonstration showcases DataLens's capabilities in effectively identifying and correcting data errors, improving data quality for downstream tasks, and promoting reproducibility in data cleaning pipelines.

==> sections/related_work.tex <==
%=====================
\section{Related Work}\label{sec:related_work}
%=====================
%
In this section, we report on the state-of-the-art techniques and tools relevant to \PaperAcronym{}.  There exist also a few research papers that tackle the data quality problem. For instance, Ramneesh et al. [7] presents a dashboard for linked data quality assessment. The dashboard leverages AI methods to evaluate and monitor the quality of linked data. While it offers novel ways to handle linked data, its scope may be limited to this specific data type and may not provide comprehensive solutions for broader data quality issues. Similarly, Blacketer et al. [8] show the application of a data quality dashboard to ensure conformance to model specifications within the European Health Data and Evidence Network (EHDEN). While the dashboard's application in a network like EHDEN underlines its potential, it might be heavily tailored to specific requirements of such a network and may not be fully applicable to other domains or data types. Gitzel et al. [9] introduces a data quality dashboard for Computerized Maintenance Management System (CMMS) data, where all equipment failures are reported. The focus on CMMS data indicates a high level of specialization, which could limit its broader applications. Additionally, being published in 2018, it might lack some of the more recent advancements in data quality management, such as deep integration with machine learning tools and processes.
There exist also some data quality dashboards from industry, such as Informatica Data Quality, Talend Data Quality, IBM InfoSphere Information Analyzer, SAS Data Quality, and DataRobot Paxata. These tools offer a variety of features designed to monitor and improve data quality. However, they also present certain challenges. Configurations for these dashboards can be complex, often requiring skilled personnel to set up and manage effectively. The integration of these tools into existing systems may require additional effort and customization, potentially leading to increased overhead and complexity. Furthermore, these tools typically require users to define various parameters, such as data sources, data profiling objectives, data quality rules, thresholds, and metrics. While this offers a high degree of flexibility, it can also place a significant burden on users, particularly those with less technical expertise in data quality management.
3	Disadvantages of Closest Prior Art
The state-of-the-art tools and methods have several shortcomings which hinder their adoption in real-world applications. In this section, we motivate for the development through elaborating on the major shortcomings of the state-of-the-art methods and tools, which include: 
•	Limited Data Quality Management: Existing patents focus on data visualization and fail to address critical aspects of data quality management, such as automated data profiling, validation, and correction.
•	Outdated Approaches: The patents broadly rely on outdated approaches which do not consider recent advancements in data quality management. 
•	Dependence on User Understanding: The patents rely heavily on a user's understanding and definition of data quality, which can vary considerably and may not cover all aspects of data quality.
•	Limited Scope: Some research papers present methodologies that might be limited to specific data types or domains, preventing broader application. 
•	Complexity and User Burden: Commercial data quality dashboards can be complex to configure and integrate into existing systems, requiring skilled personnel and potentially increasing overhead. 

The proposed invention addresses the shortcomings of existing data quality management tools by providing an automated, interactive dashboard. It leverages advanced algorithms and ML for automated data profiling, validation, error detection, and correction. The system integrates with common ML tracking tools like MLflow and Delta Lake, enabling robust data management and tracking of changes over time. Additionally, it generates detailed DataSheets for transparency and supports iterative cleaning for continuous improvement. The role of the data owner is streamlined, reducing their technical burden while maximizing their input value, making this solution efficient, effective, and user-friendly. Moreover, it supports the “user-in-the-loop” strategy via enabling users to add their rules or to define certain data samples to be corrupted. Finally, the iterative cleaning strategy enables the generation of repair data versions well-suited for ML training and serving. 



%In fact, there are several patents that tackled the problem of data visualization and data quality. For instance, the patent by Kumar et al. [3] focuses on visualizing data of enterprise assets based on insights drawn from a knowledge graph. Similarly, the patent by Barbouche et al. [4] emphasizes comparing medical data in an automated system using a variety of visualization tools. While these approaches provide valuable insights into the relationships and dependencies between different assets, it could fall short in areas of data quality management. The patents do not explicitly mention automated data profiling, validation, or correction, which are crucial aspects in maintaining high-quality data. Additionally, the reliance on knowledge graphs could limit its applicability for datasets where complex relationships are not the primary concern.

%The patent by Al Za’noun et al. [5] introduces a system that performs basic data checks and uses a cost model to provide a data quality scorecard. However, its approach might be considered somewhat outdated as it was filed in 2015, and there have been significant advancements in data quality management since then. Moreover, it may lack the sophistication of automated rule extraction, automated data correction, and machine learning model integration, which are crucial for modern, efficient data quality management. The patent by Yamashita et al. [6] involves a system that receives a data quality requirement from a user. While this user-centric approach is commendable, it may rely heavily on the user's understanding and definition of data quality, which could vary and might not address all aspects of data quality. Furthermore, it doesn't mention features like automated data profiling, error detection, and correction or the integration with machine learning tracking tools, which can streamline and improve the data quality management process.
